Learning from straggler clients in federated learning

How well do existing federated learning algorithms learn from client devices that return model updates with a significant time delay? Is it even possible to learn effectively from clients that report back minutes, hours, or days after being scheduled? We answer these questions by developing Monte Carlo simulations of client latency that are guided by real-world applications. We study synchronous optimization algorithms like FedAvg and FedAdam as well as the asynchronous FedBuff algorithm, and observe that all these existing approaches struggle to learn from severely delayed clients. To improve upon this situation, we experiment with modifications, including distillation regularization and exponential moving averages of model weights. Finally, we introduce two new algorithms, FARe-DUST and FeAST-on-MSG, based on distillation and averaging, respectively. Experiments with the EMNIST, CIFAR-100, and StackOverflow benchmark federated learning tasks demonstrate that our new algorithms outperform existing ones in terms of accuracy for straggler clients, while also providing better trade-offs between training time and total accuracy.

==> Sections/convergence.tex <==
\section{Proof of Convergence Rate of \feast{} Algorithm}\label{sec:convergence}
Recall the notation used in FeASTon-MSG Algorithm, for any iteration $t=1,2,\ldots...,T$, the subset of sampled clients are defined as $\mathcal{C}_t\subset[m]$ of size $|\mathcal{C}_t|=B^{+}$. Each sampled client $c\in\mathcal{C}_t$ runs $T_l$ iterations of local SGD and returns the local update:
\begin{equation}
\Delta_t^{c}=\eta_l\sum_{k=0}^{T_l-1} g_{c}\left(w_{t,k}^{c}\right),
\end{equation} 
where $w_{t,0}^{c}=w_t$ and $w_{t,k}^{c}=w_{t,k-1}^{c}-\eta_l g_{c}\left(w_{t,k-1}^{c}\right)$. Furthermore, $g_{c}\left(w_{t,k}^{c}\right)$ is the stochastic gradient of the local function $F_c$ computed from the local dataset at client $c\in\mathcal{C}_t$. The main model $w_{t}$ is updated as follows:
\begin{equation}~\label{eqn:global_update}
w_{t+1}=w_t-\frac{\eta_g}{B}\Delta_{t},
\end{equation} 
where $\Delta_t=\sum_{c\in\mathcal{C}^{\text{fast}}_t}\Delta_t^{c}$ denotes the summation of the local updates for the fastest $B\leq B^{+}$ clients, where $\mathcal{C}^{\text{fast}}_t\subset\mathcal{C}_t$ with $|\mathcal{C}_t^{\text{fast}}|=B$. The server keeps aggregating the local updates from the slow clients till for additional duration $\tau_{\max}$ as follows:
\begin{equation}~\label{eq:Delta+}
\Delta_t^{+}=\Delta_t+\sum_{c\in\mathcal{C}_{t}^{\text{slow}}}\Delta_t^{c},
\end{equation}
where $\mathcal{C}_t^{\text{slow}}\subseteq \mathcal{C}_t\setminus\mathcal{C}_t^{\text{fast}}$ and $B_t^{+}=|\mathcal{C}_t^{\text{fast}}|+|\mathcal{C}_t^{\text{slow}}|$. The server updates the auxiliary global model $a_{t+1}$ as follows:
\begin{equation}
a_{t+1}=\beta \left(a_t-\frac{\eta_a}{B_t^{+}}\Delta_t^{+}\right)+(1-\beta)w_{t+1}^{+},
\end{equation}
where $w_{t+1}^{+}=w_{t}-\frac{\eta_g}{B_{t}^{+}}\Delta_{t}^{+}$ and $\beta\in[0,1]$ is the EMA parameter. For simplicity, let $\eta_a=\eta_g$. Thus, we can reformulate the update of the auxiliary model $a_{t+1}$ as follows:
\begin{equation}~\label{eq:aux_update}
a_{t+1}=a_{t}-(1-\beta)(a_t-w_t)-\frac{\eta_g}{B_t^{+}}\Delta_{t}^{+}.
\end{equation}
We consider the following assumptions on the gradients and the functions throughout the analysis which are common in FL analysis.

\begin{assumption}[Smooth functions]~\label{assump:lipschitz} For each client $i\in[m]$, the loss function $F_i$ is $L$-smooth, i.e., the gradient is Lipschitz continuous:
\begin{equation}
\|\nabla F_i(w)-\nabla F_i(w')\|\leq L\|w-w'\|\qquad\forall w,w'\in\mathbb{R}^{d}.
\end{equation}
\end{assumption}


\begin{assumption}[Bounded gradients]~\label{assump:bound_gradient}
For all $i\in[m]$, the gradient $\nabla F_{i}(w)$ satisfies $\|\nabla F_i(w)\|^2\leq G^2$
\end{assumption}

%
\begin{assumption}[Stochastic gradients]~\label{assump:gradient}
For all $i\in[m]$, the stochastic gradient $g_{i}(w)$ is unbiased and has bounded variance, i.e., there exist finite $\sigma_{l}^2$ such that
\begin{enumerate}
\item {\it Unbiased: } $\mathbb{E}[g_i(w)] = \nabla F_i(w)\quad\forall w\in\mathbb{R}^{d}$.
\item {\it Bounded variance: } $\mathbb{E}\|g_i(w)-\nabla F_i(w)\|^2 \leq \sigma_{l}^2 \quad\forall w\in\mathbb{R}^{d}$. 
 \end{enumerate}
\end{assumption}


\begin{assumption}[Additional time]~\label{assump:time} The additional time $\tau_{\max}$ that the server keeps updating the $\Delta_{t}^{+}$ is sufficient to add all sampled clients in each $t\in[T]$. Hence, $B_t^{+}=|\mathcal{C}_t^{\text{fast}}|+|\mathcal{C}_t^{\text{slow}}|=|\mathcal{C}_t|=B^{+}$.
\end{assumption}
Note that Assumption~\ref{assump:time} is to simplify the analysis by fixing the value $B_t^{+}=B^{+}$ for all $t\in[T]$. However, our analysis is valid for general values of $\lbrace B_t^{+} \rbrace$. Our main convergence result is as follows.

\begin{theorem}~\label{thm:convergecne} If we run \feast{} for $T$ iterations with $\beta\leq\frac{B}{B^{+}}$ and learning rates satisfying $\frac{\eta_g\eta_lT_l}{2}=\frac{1}{\sqrt{T}}$ and $\eta_g\geq 1$, the auxiliary model satisfies 
\begin{align}\label{nonconvex-convergence}
\frac{1}{T}\sum_{t=1}^T\mathbb{E}\|\nabla f(a_t)\|^2 &\leq  \frac{(f(a_0) - f^{*})}{\sqrt{T}}  + \left(\frac{10}{\sqrt{T}}+\frac{2.5L^2}{T}\right)\left(\sigma_l^2+G^2\right)
\end{align}
\end{theorem}

We first prove some useful lemmas before proceeding in the proof of Theorem~\ref{thm:convergecne}.

\begin{lemma}\label{lem:recursion_gap} For any iteration $t\in[T]$, we have that
\begin{equation}~\label{eq:recursion_formula}
a_{t+1}-w_{t+1}=\eta_g\sum_{k=0}^{t}\beta^{k}\left[\left(\frac{1}{B}-\frac{1}{B^{+}}\right)\Delta_{t-k}-\frac{1}{B^{+}}\Delta_{t-k}^{\text{slow}}\right],
\end{equation}
\begin{equation}~\label{eq:recursion_expectation}
\mathbb{E}\left[a_{t+1}-w_{t+1}\right]=0,
\end{equation}
where the expectation is w.r.t. client sampling, stochastic gradient, and iterations history. The term $\Delta_{t-k}^{\text{slow}}=\sum_{c\in\mathcal{C}_{t-k}^{\text{slow}}}\Delta_{t-k}^{c}$ the summation of local updates of the slow clients at iteration $t-k$, and $\Delta_{t-k}=\sum_{c\in\mathcal{C}_{t-k}^{\text{fast}}}\Delta_{t-k}^{c}$ the summation of local updates of the fast clients at iteration $t-k$.
\end{lemma}


\begin{lemma}\label{lem:reduced-variance} For any iteration $t\in[T]$, and local iteration $l\in[T_l]$, we have that
\begin{equation}
\mathbb{E}\left[\left\|g_{c}\left(w_{t,l}^{c}\right)\right\|^2\right]\leq \sigma_l^2+G^2,
\end{equation}
where the expectation is taken w.r.t. client sampling, the randomness of the stochastic gradient $g_c$, and the history of the iterations.
\end{lemma}

\begin{lemma}\label{lem:gap_aux-global} For any iteration $t\in[T]$, we have that 
\begin{equation}
\mathbb{E}\left[\|a_t-w_t\|^2\right]\leq \frac{4\eta_g^2\eta_l^2T_l^2}{(1-\beta)^2}\left(1-\frac{B}{B^{+}}\right)^2\left(\sigma_l^2 +  G^2\right),
\end{equation} 
where the expectation is taken w.r.t. client sampling, the randomness of the stochastic gradient $g_i$, and the history of the iterations.
\end{lemma}
Observe that Lemma~\ref{lem:gap_aux-global} bounds the distance between the auxiliary model $a_{t}$ (that has additional updates from slow clients) and the global model $w_t$. In a special case when $B^{+}=B$, i.e., there is no slow clients, we can verify that $a_t=w_t$. By plugging $B^{+}=B$, Lemma~\ref{lem:gap_aux-global} shows that \noteEA{$\|a_t-w_t\|^2 = 0$ a.s.} By carefully choosing local learning rate $\eta_l$, global learning rate $\eta_g$, and EMA parameter $\beta$, we can guarantee that $\|a_t-w_t\|$ doesn't diverge over the iterations.


The proof of Lemma~\ref{lem:recursion_gap} is presented in Section~\ref{sec:proofs-lemma_recursion_gap}. The proof of Lemma~\ref{lem:reduced-variance} is presented in Section~\ref{sec:proofs-lemma_reduced} and the proof of Lemma~\ref{lem:gap_aux-global} is presented in Section~\ref{sec:proofs-lemma_gap_aux}.


\subsection{Proof of Theorem~\ref{thm:convergecne}}\label{sec:non-convex}

%
Using the $L$-smoothness of $f$ (which follows from the $L$-smoothness of $F_1,\ldots,F_m$), we get that
\begin{equation}~\label{eq:loss_bound}
\begin{aligned}
f(a_{t+1}) &\leq f(a_{t}) + \left\langle \nabla f(a_t), a_{t+1} - a_{t} \right\rangle + \frac{L}{2}\left\|a_{t+1} - a_{t}\right\|^2 \nonumber \\
&= f(a_t) \underbrace{-\left\langle \nabla f(a_t),(1-\beta)(a_t-w_t)+\frac{\eta_g}{B^{+}}\Delta^{+}_t\right\rangle}_{T_1} +\underbrace{\frac{L}{2} \left\| (1-\beta)(a_t-w_t)+\frac{\eta_g}{B^{+}}\Delta^{+}_t \right\|^2}_{T_2}
\end{aligned}
\end{equation}
We first bound the term $T_1$ and then $T_2$. Taking expectation w.r.t.\ the randomness of stochastic gradients, client sampling, iterations history and using the conditional expectation ($\mathbb{E}[\cdot]=\mathbb{E}_{\mathcal{H}}\mathbb{E}_{\mathcal{C}_t\subset[m]}\mathbb{E}_{g_c|\mathcal{C}_t,\mathcal{H}}[\cdot]$), we have that
\begin{equation}
\begin{aligned}
\mathbb{E}\left[T_1\right]&=-\mathbb{E}\left[\left\langle \nabla f(a_t),(1-\beta)(a_t-w_t)+\frac{\eta_g}{B^{+}}\Delta^{+}_t\right\rangle\right]\\
&=(1-\beta)\mathbb{E}_{\mathcal{H}}\left[\underbrace{-\left\langle \nabla f(a_t),(a_t-w_t)\right\rangle}_{T_3}\right]-\mathbb{E}_{\mathcal{H}}\left[\left\langle \nabla f(a_t),\frac{\eta_g\eta_l}{B^{+}}\mathbb{E}_{\mathcal{C}_t,g_c}\left[\sum_{c\in\mathcal{C}_t}\sum_{l=0}^{T_l-1}g_c(w_{t,l}^{c})\right]\right\rangle\right]\\
&=(1-\beta)\mathbb{E}_{\mathcal{H}}\left[T_3\right]+\eta_g\eta_l\mathbb{E}_{\mathcal{H}}\left[\underbrace{-\left\langle \nabla f(a_t),\frac{1}{m}\sum_{i=1}^{m}\sum_{k=0}^{T_l-1}\nabla F_i(w_{t,k}^{i})\right\rangle}_{T_4}\right]\\
&=(1-\beta)\mathbb{E}_{\mathcal{H}}\left[T_3\right]+\eta_g\eta_l\mathbb{E}_{\mathcal{H}}\left[T_4\right],
\end{aligned}
\end{equation}
We bound the term $\mathbb{E}\left[T_4\right]$ as follows.
\begin{align}
\mathbb{E}\left[T_4\right]&=-\mathbb{E}_{\mathcal{H}}\left[\left\langle \nabla f(a_t),\frac{1}{m}\sum_{i=1}^{m}\sum_{l=0}^{T_l-1}\nabla F_i(w_{t,l}^{i})\right\rangle\right]\nonumber\\ 
&=\sum_{l=1}^{T_l-1}\mathbb{E}\left[-\left\langle \nabla f(a_t),\frac{1}{m}\sum_{i=1}^{m}\nabla F_i(w_{t,l}^{i})\right\rangle\right]\nonumber\\
&\stackrel{\text{(a)}}{=}\frac{1}{2}\sum_{l=1}^{T_l-1}\mathbb{E}\left[\left\|\nabla f(a_t)-\frac{1}{m}\sum_{i=1}^{m}\nabla F_i(w_{t,l}^{i})\right\|^2-\left\|\nabla f(a_t)\right\|^2-\left\|\frac{1}{m}\sum_{i=1}^{m}\nabla F_i(w_{t,l}^{i})\right\|^2\right]\nonumber\\
&\stackrel{\text{(b)}}{=}\frac{1}{2}\sum_{l=1}^{T_l-1}\mathbb{E}\left[\left\|\frac{1}{m}\sum_{i=1}^{m}\nabla F_i(a_t)-\frac{1}{m}\sum_{i=1}^{m}\nabla F_i(w_{t,l}^{i})\right\|^2-\left\|\nabla f(a_t)\right\|^2-\left\|\frac{1}{m}\sum_{i=1}^{m}\nabla F_i(w_{t,l}^{i})\right\|^2\right]\nonumber\\
&\stackrel{\text{(c)}}{\leq}\frac{1}{2}\sum_{l=1}^{T_l-1}\mathbb{E}\left[\frac{1}{m}\sum_{i=1}^{m}\left\|\nabla F_i(a_t)-\nabla F_i(w_{t,l}^{i})\right\|^2-\left\|\nabla f(a_t)\right\|^2\right]\nonumber\\
&=\frac{1}{2}\sum_{k=1}^{T_l-1}\mathbb{E}\left[\frac{1}{m}\sum_{i=1}^{m}\left\|\nabla F_i(a_t)-\nabla F_i(w_t)+\nabla F_i(w_t)-\nabla F_i(w_{t,l}^{i})\right\|^2-\left\|\nabla f(a_t)\right\|^2\right]\nonumber\\
&\leq\frac{1}{2}\sum_{l=1}^{T_l-1}\mathbb{E}\left[\frac{2}{m}\sum_{i=1}^{m}\left(\left\|\nabla F_i(a_t)-\nabla F_i(w_t)\right\|^2+\left\|\nabla F_i(w_t)-\nabla F_i(w_{t,l}^{i})\right\|^2\right)-\left\|\nabla f(a_t)\right\|^2\right]\nonumber\\
&\stackrel{\text{(d)}}{\leq}\frac{1}{2}\sum_{l=1}^{T_l-1}\mathbb{E}\left[\frac{2}{m}\sum_{i=1}^{m}\left(L^2\left\|a_t-w_t\right\|^2+L^2\left\|w_t-w_{t,l}^{i}\right\|^2\right)-\left\|\nabla f(a_t)\right\|^2\right]\nonumber\\
&=T_lL^2 \mathbb{E}\left[\left\|a_t-w_t\right\|^2\right]+L^2\sum_{l=1}^{T_l-1}\frac{1}{m}\sum_{i=1}^{m}\mathbb{E}\left[\left\|w_t-w_{t,l}^{i}\right\|^2\right]-\frac{T_l}{2}\mathbb{E}\left[\left\|\nabla f(a_t)\right\|^2\right]\nonumber\\
&=T_lL^2 \mathbb{E}\left[\left\|a_t-w_t\right\|^2\right]+L^2\sum_{l=1}^{T_l-1}\frac{1}{m}\sum_{i=1}^{m}\mathbb{E}\left[\left\|\eta_l\sum_{j=0}^{l-1}g_i(w_{t,j}^{i})\right\|^2\right]-\frac{T_l}{2}\mathbb{E}\left[\left\|\nabla f(a_t)\right\|^2\right]\nonumber\\
&\leq T_lL^2 \mathbb{E}\left[\left\|a_t-w_t\right\|^2\right]+\eta_l^2L^2\sum_{l=1}^{T_l-1}\frac{1}{m}\sum_{i=1}^{m}\sum_{j=0}^{l-1}k\mathbb{E}\left[\left\|g_i(w_{t,j}^{i})\right\|^2\right]-\frac{T_l}{2}\mathbb{E}\left[\left\|\nabla f(a_t)\right\|^2\right]\nonumber\\
&\leq T_lL^2 \mathbb{E}\left[\left\|a_t-w_t\right\|^2\right]+\eta_l^2T_l^3L^2\left(\sigma_l^2+G^2\right)-\frac{T_l}{2}\mathbb{E}\left[\left\|\nabla f(a_t)\right\|^2\right],
\end{align}
where step (a) follows from the equality $-\langle a,b\rangle=1/2\left(\|a-b\|^2-\|a\|^2-\|b\|^2\right)$. Step (b) follows from the fact that $f(w)=\frac{1}{m}\sum_{i=1}^{m}F_i(w)$, and step (c) follows from Jensen's inequality. Step (d) follows from Assumption~\ref{assump:lipschitz} of Lipschitzness. Now, we bound the term $\mathbb{E}_{\mathcal{H}}\left[T_3\right]$.
\begin{align}
\mathbb{E}_{\mathcal{H}}\left[T_3\right] &= - \mathbb{E}_{\mathcal{H}}\left[\left\langle \nabla f(a_t),(a_t-w_t)\right\rangle\right] \nonumber \\
&= - \mathbb{E}_{\mathcal{H}}\left[\left\langle \nabla f(a_t)-\nabla f(w_t),(a_t-w_t)\right\rangle\right] - \mathbb{E}_{\mathcal{H}}\left[\left\langle \nabla f(w_t),(a_t-w_t)\right\rangle\right] \nonumber\\
&\stackrel{\text{(a)}}{\leq} L\mathbb{E}\left[\|a_t-w_t\|^2\right]- \mathbb{E}_{\mathcal{H}}\left[\left\langle \nabla f(w_t),(a_t-w_t)\right\rangle\right]\nonumber\\
&\stackrel{\text{(b)}}{=}L\mathbb{E}\left[\|a_t-w_t\|^2\right]-\eta_g\sum_{k=0}^{t-1}\beta^{k} \mathbb{E}_{\mathcal{H}}\left[\left\langle \nabla f(w_t),\left[\left(\frac{1}{B}-\frac{1}{B^{+}}\right)\Delta_{t-k}-\frac{1}{B^{+}}\Delta_{t-k}^{\text{slow}}\right]\right\rangle\right]\nonumber\\
&=L\mathbb{E}\left[\|a_t-w_t\|^2\right]+\eta_g\sum_{k=0}^{t-1}\beta^{k}\left(\frac{1}{B}-\frac{1}{B^{+}}\right) \mathbb{E}_{\mathcal{H}}\left[\underbrace{-\left\langle \nabla f(w_t),\Delta_{t-k}\right\rangle}_{T_{t-k}}\right]\nonumber\\
&\qquad+\eta_g\sum_{k=0}^{t-1}\beta^{k}\frac{1}{B^{+}}\mathbb{E}_{\mathcal{H}}\left[\underbrace{\left\langle \nabla f(w_t),\Delta_{t-k}^{\text{slow}}\right\rangle}_{T_{t-k,2}}\right]\nonumber\\
&=L\mathbb{E}\left[\|a_t-w_t\|^2\right]+\eta_g\sum_{k=0}^{t-1}\beta^k\left(\mathbb{E}_{\mathcal{H}}\left[T_{t-k}\right]+\mathbb{E}_{\mathcal{H}}\left[T_{t-k,2}\right]\right)
\end{align}
where step (a) is obtained from Assumption~\ref{assump:lipschitz} and the fact that $\langle a,b\rangle\leq \|a\|\|b\|$. Step (b) follows from Lemma~\ref{lem:recursion_gap}.

\begin{align}
\mathbb{E}_{\mathcal{H}}\left[T_{t-k}\right] &= - \mathbb{E}_{\mathcal{H}}\left[\left\langle \nabla f(w_t),\Delta_{t-k}\right\rangle\right]\nonumber\\
&= - \eta_l\sum_{l=0}^{T_l-1}\mathbb{E}\left[\sum_{c\in\mathcal{C}_{t-k}^{\text{fast}}}\left\langle \nabla f(w_t),g_c(w_{t-k,l}^c)\right\rangle\right]\nonumber\\
&=\eta_l\sum_{l=0}^{T_l-1}\Bigg(\mathbb{E}\left[-\sum_{c\in\mathcal{C}_{t-k}^{\text{fast}}}\left\langle \nabla f(w_t)-\nabla f(w_{t-k}),g_c(w_{t-k,l}^c)\right\rangle\right]\nonumber\\
&\qquad-\mathbb{E}\left[\sum_{c\in\mathcal{C}_{t-k}^{\text{fast}}}\left\langle \nabla f(w_{t-k}),g_c(w_{t-k,l}^c)\right\rangle\right]\Bigg)\nonumber\\
&\stackrel{\text{(a)}}{=}\eta_l\sum_{c\in\mathcal{C}_{t-k}^{\text{fast}}}\sum_{l=0}^{T_l-1}\sqrt{L^2\mathbb{E}\left[\|w_t-w_{t-k}\|^2\right]\mathbb{E}\left[\|g_c(w_{t-k,l}^c)\|^2\right]}\nonumber\\
&\qquad -\eta_l \frac{B}{m} \sum_{l=0}^{T_l-1}\sum_{i=1}^{m}\mathbb{E}\left[\langle\nabla f(w_{t-k}),\nabla F_i(w_{t-k,l}^{i})\rangle\right]
\end{align}

Now, we bound the term $\mathbb{E}[T_2]$:
\begin{align}
\mathbb{E}\left[T_2\right]&=\mathbb{E}\left[\left\| (1-\beta)(a_t-w_t)+\frac{\eta_g}{B^{+}}\Delta^{+}_t \right\|^2\right]\nonumber\\
&\leq 2 (1-\beta)^2\mathbb{E}\left[\left\| (a_t-w_t)\right\|^2\right]+2\mathbb{E}\left[\left\|\frac{\eta_g}{B^{+}}\Delta^{+}_t \right\|^2\right]\nonumber\\
&= 2 (1-\beta)^2\mathbb{E}\left[\left\| (a_t-w_t)\right\|^2\right]+2\frac{\eta_g^2}{\left(B^{+}\right)^2}\mathbb{E}\left[\left\|\sum_{c\in\mathcal{C}_t}\sum_{l=0}^{T_l-1}\eta_lg_c(w_{t,l}^{c}) \right\|^2\right]\nonumber\\
&\leq2 (1-\beta)^2\mathbb{E}\left[\left\| (a_t-w_t)\right\|^2\right]+2\frac{\eta_g^2\eta_l^2T_l}{B^{+}}\sum_{l=0}^{T_l-1}\mathbb{E}_{\mathcal{C}_t}\left[\sum_{c\in\mathcal{C}_t}\mathbb{E}_{g_c|c}\left[\|g_c(w_{t,l}^{c})\|^2\right]\right]\nonumber\\
&\leq 2 (1-\beta)^2\mathbb{E}\left[\left\| (a_t-w_t)\right\|^2\right]+2\frac{\eta_g^2\eta_l^2T_l}{B^{+}}\sum_{l=0}^{T_l-1}\mathbb{E}_{\mathcal{C}_t}\left[\sum_{c\in\mathcal{C}_t}\left(\sigma_l^2+G^2\right)\right]\nonumber\\
&= 2 (1-\beta)^2\mathbb{E}\left[\left\| (a_t-w_t)\right\|^2\right]+2\eta_g^2\eta_l^2T_l^2\left(\sigma_l^2+G^2\right),
\end{align}
where the first and the second inequalities are obtained from Jensen's inequality and the third inequality is obtained from Lemma~\ref{lem:reduced-variance}. Thus, we get that
\begin{equation}
\begin{aligned}
f(a_{t+1})\leq f(a_t)-A_1\mathbb{E}\left[\|\nabla f(a_t)\|^2\right]+A_2\mathbb{E}\left[\left\|a_t-w_t\right\|^2\right]+A_3\left(\sigma_l^2+G^2\right),
\end{aligned}
\end{equation} 
where $A_1=\frac{\eta_g\eta_lT_l}{2}$ and $A_2=\eta_g\eta_lT_lL^2+2(1-\beta)^2$. The term $A_3=\eta_g\eta_l^3T_l^3L^2+2\eta_g^2\eta_l^2T_l^2$. Thus, we have that
\begin{equation}
\begin{aligned}
\frac{1}{T}\sum_{t=0}^{T-1}\mathbb{E}\left[\|\nabla f(a_t)\|^2\right]&\leq \frac{f(a_0)-f(a_T)}{T A_1}+\frac{A_2}{A_1}\frac{1}{T}\sum_{t=0}^{T-1}\mathbb{E}\left[\left\|a_t-w_t\right\|^2\right]+\frac{A_3}{A_1}\left(\sigma_l^2+G^2\right)\\
&\stackrel{\text{(a)}}{\leq} \frac{f(w_0)-f^{*}}{T A_1}+\frac{A_2}{A_1}\frac{1}{T}\sum_{t=0}^{T-1}\mathbb{E}\left[\left\|a_t-w_t\right\|^2\right]+\frac{A_3}{A_1}\left(\sigma_l^2+G^2\right)\\
&\stackrel{\text{(b)}}{\leq} \frac{f(w_0)-f^{*}}{T A_1}+\frac{A_2}{A_1}\frac{4\eta_g^2\eta_l^2T_l^2}{(1-\beta)^2}\left(1-\frac{B}{B^{+}}\right)^2\left(\sigma_l^2+G^2\right)+\frac{A_3}{A_1}\left(\sigma_l^2+G^2\right)\\
&\stackrel{\text{(c)}}{\leq}\frac{f(w_0)-f^{*}}{T A_1}+\left(\frac{A_2}{A_1}\times 4\eta_g^2\eta_l^2T_l^2+\frac{A_3}{A_1}\right)\left(\sigma_l^2+G^2\right)\\
&\stackrel{\text{(d)}}{\leq}\frac{f(w_0)-f^{*}}{T A_1}+\left(8A_1^2L_2+16A_1+\frac{2A_1^2}{\eta_g^2} L^2+4A_1\right)\left(\sigma_l^2+G^2\right)\\
&\stackrel{\text{(e)}}{\leq}\frac{f(w_0)-f^{*}}{T A_1}+\left(10A_1+2.5A_1^2L^2\right)\left(\sigma_l^2+G^2\right)\\
&\stackrel{\text{(f)}}{\leq}\frac{f(w_0)-f^{*}}{\sqrt{T}}+\left(\frac{10}{\sqrt{T}}+\frac{2.5L^2}{T}\right)\left(\sigma_l^2+G^2\right),
\end{aligned}
\end{equation}
where step (a) follows from the fact that $a_0=w_0$ and $f^{*}\leq f(a_T)$ is the optimal loss. Step (b) follows from Lemma~\ref{lem:gap_aux-global}. Step (c) follows from choosing $\beta =\frac{B}{B^{+}}$ and step (d) follows from the fact that $(1-\beta)^2\leq 1$. Step (e) is obtained from choosing $\eta_g\geq 1$ and step (f) is obtained by choosing $A_1=\frac{\eta_g\eta_lT_l}{2}=\frac{1}{\sqrt{T}}$. 


\subsection{Proof of Lemma~\ref{lem:recursion_gap}}~\label{sec:proofs-lemma_recursion_gap}

\begin{proof}[Proof of Lemma~\ref{lem:recursion_gap}] From the update rule of the auxiliary model $a_{t+1}$ in~\eqref{eq:aux_update}, we have that
\begin{equation}~\label{eq:recursion_app}
\begin{aligned}
a_{t+1}-w_{t+1}&=a_t-(1-\beta)(a_t-w_t)-\frac{\eta_g}{B^{+}}\Delta_t^{+}-\left(w_t-\frac{\eta_g}{B}\Delta_t\right)\\
&\stackrel{\text{(a)}}{=}\beta(a_t-w_t)-\frac{\eta_g}{B^{+}}\Delta_t^{\text{slow}}+\left(\frac{\eta_g}{B}-\frac{\eta_g}{B^{+}}\right)\Delta_t,
\end{aligned}
\end{equation}
where (a) follows from~\eqref{eq:aux_update}, where $\Delta_t^{\text{slow}}=\sum_{c\in\mathcal{C}_t^{\text{slow}}}\Delta_t^{c}$. Note that $a_0=w_0$, and hence, from induction, we can show that
\begin{equation}
\begin{aligned}
a_{t+1}-w_{t+1}&=\eta_g\sum_{k=0}^{t}\beta^{k}\left[\left(\frac{1}{B}-\frac{1}{B^{+}}\right)\Delta_{t-k}-\frac{1}{B^{+}}\Delta_{t-k}^{\text{slow}}\right].
\end{aligned}
\end{equation}
This proves~\eqref{eq:recursion_formula}. Now, we prove~\eqref{eq:recursion_expectation} by induction. For the base case when $t=0$, we have that $a_0=w_0$, and hence, $\mathbb{E}\left[a_0-w_0\right]=0$. Suppose~\eqref{eq:recursion_expectation} is true at iteration $t$. From~\eqref{eq:recursion_app}, we have that:
\begin{equation}
\begin{aligned}
\mathbb{E}\left[a_{t+1}-w_{t+1}\right]&=\mathbb{E}\left[\beta(a_t-w_t)-\frac{\eta_g}{B^{+}}\Delta_t^{\text{slow}}+\left(\frac{\eta_g}{B}-\frac{\eta_g}{B^{+}}\right)\Delta_t\right]\\
&=\beta\mathbb{E}\left[(a_t-w_t)\right]-\frac{\eta_g}{B^{+}}\mathbb{E}\left[\Delta_t^{\text{slow}}\right]+\left(\frac{\eta_g}{B}-\frac{\eta_g}{B^{+}}\right)\mathbb{E}\left[\Delta_t\right]\\
&\stackrel{\text{(a)}}{=}0-\frac{\eta_g}{B^{+}}\mathbb{E}\left[\sum_{c\in\mathcal{C}_t^{\text{slow}}}\sum_{l=0}^{T_l-1}g_c(w_{t,l}^{c})\right]+\left(\frac{\eta_g}{B}-\frac{\eta_g}{B^{+}}\right)\mathbb{E}\left[\sum_{c\in\mathcal{C}_t^{\text{fast}}}\sum_{l=0}^{T_l-1}g_c(w_{t,l}^{c})\right]\\
&\stackrel{\text{(b)}}{=}-\frac{\eta_g}{B^{+}}\mathbb{E}_{\mathcal{H}}\left[\mathbb{E}_{\mathcal{C}_t\subset[m]}\left[\sum_{c\in\mathcal{C}_t^{\text{slow}}}\mathbb{E}_{g_c|\mathcal{C}_t,\mathcal{H}}\left[\sum_{l=0}^{T_l-1}g_c(w_{t,l}^{c})\right]\right]\right]\\
&\qquad+\left(\frac{\eta_g}{B}-\frac{\eta_g}{B^{+}}\right)\mathbb{E}_{\mathcal{H}}\left[\mathbb{E}_{\mathcal{C}_t\subset[m]}\left[\sum_{c\in\mathcal{C}_t^{\text{fast}}}\mathbb{E}_{g_c|\mathcal{C}_t,\mathcal{H}}\left[\sum_{l=0}^{T_l-1}g_c(w_{t,l}^{c})\right]\right]\right]\\
&\stackrel{\text{(c)}}{=}-\frac{\eta_g}{B^{+}}\mathbb{E}_{\mathcal{H}}\left[\mathbb{E}_{\mathcal{C}_t\subset[m]}\left[\sum_{c\in\mathcal{C}_t^{\text{slow}}}\sum_{l=0}^{T_l-1}\nabla F_c(w_{t,l}^{c})\right]\right]\\
&\qquad+\left(\frac{\eta_g}{B}-\frac{\eta_g}{B^{+}}\right)\mathbb{E}_{\mathcal{H}}\left[\mathbb{E}_{\mathcal{C}_t\subset[m]}\left[\sum_{c\in\mathcal{C}_t^{\text{fast}}}\sum_{l=0}^{T_l-1}\nabla F_c(w_{t,l}^{c})\right]\right]\\
&\stackrel{\text{(d)}}{=}-\frac{\eta_g}{B^{+}}\mathbb{E}_{\mathcal{H}}\left[\frac{B^{+}-B}{m}\sum_{i=1}^{m}\sum_{l=0}^{T_l-1}\nabla F_i(w_{t,l}^{i})\right]+\left(\frac{\eta_g}{B}-\frac{\eta_g}{B^{+}}\right)\mathbb{E}_{\mathcal{H}}\left[\frac{B}{m}\sum_{i=1}^{m}\sum_{l=0}^{T_l-1}\nabla F_i(w_{t,l}^{i})\right]\\
&=\eta_g\mathbb{E}_{\mathcal{H}}\left[\frac{1}{m}\sum_{i=1}^{m}\sum_{l=0}^{T_l-1}\nabla F_i(w_{t,l}^{i})\right]\left(B\left(\frac{1}{B}-\frac{1}{B^{+}}\right)-\frac{B^{+}-B}{B^{+}}\right)=0
\end{aligned}
\end{equation} 
where (a) follows from induction and (b) from the total law of expectation. Step (c) follows from Assumption~\ref{assump:gradient} of unbiased gradient and (d) from uniform sampling of clients at each iterations. 
This completes the proof of Lemma~\ref{lem:recursion_gap}.
\end{proof}


\subsection{Proof of Lemma~\ref{lem:reduced-variance}}\label{sec:proofs-lemma_reduced}


\begin{proof}[Proof of Lemma~\ref{lem:reduced-variance}]
\begin{equation}
\begin{aligned}
\mathbb{E}\left[\|g_c\left(w_{t,l}^{c}\right)\|^2\right]&=\mathbb{E}\left[\|g_c\left(w_{t,l}^{c}\right)-\nabla F_c\left(w_{t,l}^{c}\right)+\nabla F_c\left(w_{t,l}^{c}\right)\|^2\right]\\
&\stackrel{\text{(a)}}{=}\mathbb{E}_{c\sim[m]}\left[\mathbb{E}_{g_c|c}\left[\|g_c\left(w_{t,l}^{c}\right)-\nabla F_c\left(w_{t,l}^{c}\right)+\nabla F_c\left(w_{t,l}^{c}\right)\|^2\right]\right]\\
&\stackrel{\text{(b)}}{=}\mathbb{E}_{c\sim[m]}\left[\mathbb{E}_{g_c|c}\left[\|g_c\left(w_{t,l}^{c}\right)-\nabla F_c\left(w_{t,l}^{c}\right)\|^2+\|\nabla F_c\left(w_{t,l}^{c}\right)\|^2\right]\right]\\
&\stackrel{\text{(c)}}{=}\sigma_l^2+G^2,
\end{aligned}
\end{equation}
where (a) follows from the law of total expectation, and (b) follows from Assumption~\ref{assump:gradient} as the gradient $g_c$ is unbiased. Step (c) follows from Assumptions~\ref{assump:gradient} and~\ref{assump:bound_gradient} of bounded variance and bounded gradients. This completes the proof of Lemma~\ref{lem:reduced-variance}.
\end{proof}



\subsection{Proof of Lemma~\ref{lem:gap_aux-global}}\label{sec:proofs-lemma_gap_aux}

\begin{proof}[Proof of Lemma~\ref{lem:gap_aux-global}] From Lemma~\ref{lem:reduced-variance}, we have that
\begin{equation}
\begin{aligned}
a_{t+1}-w_{t+1}&=\eta_g\sum_{k=0}^{t}\beta^{k}\left[\left(\frac{1}{B}-\frac{1}{B^{+}}\right)\Delta_{t-k}-\frac{1}{B^{+}}\Delta_{t-k}^{\text{slow}}\right].
\end{aligned}
\end{equation}
Let $\Gamma_t = \sum_{k=0}^{t}\beta^{k}=\frac{1-\beta^{t+1}}{1-\beta}$. Thus, we have that
\begin{equation}~\label{eq:aux_norm}
\begin{aligned}
\|a_{t+1}-w_{t+1}\|^2&=\eta_g^2\Gamma_t^2\left\|\sum_{k=0}^{t}\frac{\beta^{k}}{\Gamma_t}\left[\left(\frac{1}{B}-\frac{1}{B^{+}}\right)\Delta_{t-k}-\frac{1}{B^{+}}\Delta_{t-k}^{\text{slow}}\right]\right\|^2\\
&\stackrel{\text{(a)}}{\leq} \eta_g^2\Gamma_t^2\sum_{k=0}^{t}\frac{\beta^{k}}{\Gamma_t}\left\|\left(\frac{1}{B}-\frac{1}{B^{+}}\right)\Delta_{t-k}-\frac{1}{B^{+}}\Delta_{t-k}^{\text{slow}}\right\|^2 \text{\noteEA{combine the two steps?}}\\
&=\eta_g^2\Gamma_t\sum_{k=0}^{t}\beta^{k}\left\|\left(\frac{1}{B}-\frac{1}{B^{+}}\right)\Delta_{t-k}-\frac{1}{B^{+}}\Delta_{t-k}^{\text{slow}}\right\|^2\\
&\stackrel{\text{(b)}}{\leq}\eta_g^2\Gamma_t\sum_{k=0}^{t}\beta^{k}\left[2\left(\frac{1}{B}-\frac{1}{B^{+}}\right)^2\|\Delta_{t-k}\|^2+2\left(\frac{1}{B^{+}}\right)^2\|\Delta_{t-k}^{\text{slow}}\|^2\right],
\end{aligned}
\end{equation}
where (a) and (b) follow from Jensen's inequality. By taking the expectation w.r.t. client sampling, stochastic gradients, and the iterations history, we get:
\begin{equation}
\begin{aligned}
\mathbb{E}\left[\|\Delta_{k}\|^2\right]&=\mathbb{E}\left[\|\sum_{c\in\mathcal{C}_{k}^{\text{fast}}}\sum_{l=0}^{T_l-1}\eta_l g_c(w_{k,l}^{c})\|^2\right]\\
&\stackrel{\text{(a)}}{\leq}\eta_l^2BT_l\sum_{l=0}^{T_l}\mathbb{E}_{\mathcal{C}_k^{\text{fast}}\sim[m]}\left[\sum_{c\in\mathcal{C}_k^{\text{fast}}}\mathbb{E}_{g_c|c}\left[\|g_c(w_{k,l}^{c})\|^2\right]\right]\\
&\stackrel{\text{(b)}}{\leq}\eta_l^2BT_l\sum_{l=0}^{T_l}\mathbb{E}_{\mathcal{C}_k^{\text{fast}}\sim[m]}\left[\sum_{c\in\mathcal{C}_k^{\text{fast}}}\left(\sigma_l^2+G^2\right)\right]\\
&=\eta_l^2B^2T_l^2\left(\sigma_l^2+G^2\right),
\end{aligned}
\end{equation}
where (a) from Jensen's inequality and (b) from Lemma~\ref{lem:reduced-variance}. Similarly, we can prove that:
\begin{equation}
\begin{aligned}
\mathbb{E}\left[\|\Delta_{k}^{\text{slow}}\|^2\right]&=\mathbb{E}\left[\|\sum_{c\in\mathcal{C}_{k}^{\text{slow}}}\sum_{l=0}^{T_l-1}\eta_l g_c(w_{k,l}^{c})\|^2\right]\\
&\leq \eta_l^2(B^{+}-B)^2T_l^2\left(\sigma_l^2+G^2\right)
\end{aligned}
\end{equation}
By taking the expectation w.r.t. client sampling, stochastic gradients, and the iterations history and substituting into~\ref{eq:aux_norm}, we get that: 
\begin{equation}
\begin{aligned}
\mathbb{E}\left[\|a_{t+1}-w_{t+1}\|^2\right]&\leq2\eta_g^2\Gamma_t\sum_{k=0}^{t}\beta^{k}\left( \left(\frac{1}{B^{+}}\right)^2\mathbb{E}\left[\|\Delta_{t-k}^{\text{slow}}\|^2\right]+\left(\frac{1}{B}-\frac{1}{B^{+}}\right)^2\mathbb{E}\left[\|\Delta_{t-k}\|^2\right]\right) \\
&\leq 2\eta_g^2\Gamma_t\sum_{k=0}^{t}\beta^{k}\eta_l^2T_l^2\left(\left(\frac{1}{B^{+}}\right)^2\left(B^{+}-B\right)^2+\left(\frac{1}{B}-\frac{1}{B^{+}}\right)^2B^2\right)\left(\sigma_l^2+G^2\right)\\
&= 4\eta_g^2\Gamma_t^2\eta_l^2T_l^2\left(1-\frac{B}{B^{+}}\right)^2\left(\sigma_l^2+G^2\right)\\
&\stackrel{\text{(a)}}{\leq} 4\frac{\eta_g^2\eta_l^2T_l^2}{(1-\beta)^2}\left(1-\frac{B}{B^{+}}\right)^2\left(\sigma_l^2 + G^2\right),
\end{aligned}
\end{equation} 
where (a) follows from inequality $\Gamma_t\leq \frac{1}{(1-\beta)}$ as $\beta\in[0,1)$. This completes the proof of Lemma~\ref{lem:gap_aux-global}.
\end{proof}





==> Sections/problem_formulation.tex <==
\section{Problem Formulation}

We study the FL framework, in which a set of $m$ clients are connected to a central server to solve the optimization problem:\vspace{-0.3cm}

\begin{equation}~\label{eqn:loss}
    \min_{w\in\mathbb{R}^{d}}\frac{1}{m}\sum_{i=1}^{m}F_i\left(w\right).
\end{equation}

Here $F_i(w)=\mathbb{E}_{z\sim\mathcal{D}_i}\left[f_i(z,w)\right]$ denotes the expected loss function of the model $w$ on the $i$-th client data $\mathcal{D}_i$. The clients' datasets $\mathcal{D}_1,\ldots,\mathcal{D}_m$ may be generated from different domains and have various sizes. The goal is to obtain a global model $w^{*}$ that minimizes the loss function in Equation~\ref{eqn:loss}.

In practice, the optimization of~\pref{eqn:loss} is performed iteratively in $T$ rounds where in each round, a subset of the clients is selected to receive a copy of the global model and perform local training. After completing the updates, the clients report their local models to the central server. As discussed earlier, the processing time to receive, update, and report back the copy of the global model varies across clients due to system and data heterogeneity. This variation creates a subset of \emph{straggler clients} that take significantly longer to complete training. In the following, we propose strategies to increase the representation of straggler clients in federated models and reduce total training time.

